Evaluating Recabilities of Foundation Models: A Multi-Domain, Multi-Dataset Benchmark

Comprehensive evaluation of the recommendation capabilities of existing foundation models across diverse datasets and domains is essential for advancing the development of recommendation foundation models. In this study, we introduce RecBench-MD, a novel and comprehensive benchmark designed to assess the recommendation abilities of foundation models from a zero-resource, multi-dataset, and multi-domain perspective. Through extensive evaluations of 19 foundation models across 15 datasets spanning 10 diverse domains -- including e-commerce, entertainment, and social media -- we identify key characteristics of these models in recommendation tasks. Our findings suggest that in-domain fine-tuning achieves optimal performance, while cross-dataset transfer learning provides effective practical support for new recommendation scenarios. Additionally, we observe that multi-domain training significantly enhances the adaptability of foundation models. All code and data have been publicly released to facilitate future research.

==> Assets/Tables/multi-domain-step.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2} 

\setlength\tabcolsep{3pt}

\caption{Performance comparison in multi-domain fine-tuning scenario. We use cell background color to indicate different settings, including \rB{}, \rG{}, and \rH{}. Only AUC metric is reported due to the page limit.}\label{tab:multi-domain}

\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllllllll}
\toprule
Model & \mind{} & \microlens{} & \goodreads{} & \cds{} & \hm{} & \movielens{} & \yelp{} & \steam{} & \electronics{} & \hotelrec{} \\

% \midrule[1pt]
% \multicolumn{11}{c}{\cellcolor{bglight} \textbf{Recommendation Approach:} Prompt-based} \\
% \midrule[1pt]
\midrule
\multirow{3}{*}{\bertbase}
& \cellcolor{kbgB} 0.4963 & \cellcolor{kbgB} 0.4992 
& \cellcolor{kbgB} 0.4958 & \cellcolor{kbgB} 0.5059 
& \cellcolor{kbgB} 0.5204 & \cellcolor{kbgB} 0.4934 
& \cellcolor{kbgB} 0.4914 & \cellcolor{kbgB} 0.5002 
& \cellcolor{kbgB} 0.5037 & \cellcolor{kbgB} \textbf{0.4955} 
% & 1
\\

% \rG{}
& \cellcolor{kbgG} 0.6004 & \cellcolor{kbgG} 0.5711 
& \cellcolor{kbgG} 0.5213 & \cellcolor{kbgG} 0.5092 
& \cellcolor{kbgG} 0.6607 & \cellcolor{kbgG} \textbf{0.5675} 
& \cellcolor{kbgG} \textbf{0.5218} & \cellcolor{kbgG} 0.6189 
& \cellcolor{kbgG} \textbf{0.5091} & \cellcolor{kbgG} 0.4795
% & 8
\\

% \rH{}
& \cellcolor{kbgH} \textbf{0.7004} & \cellcolor{kbgH} \textbf{0.8019} 
& \cellcolor{kbgH} \textbf{0.5648} & \cellcolor{kbgH} \textbf{0.5653} 
& \cellcolor{kbgH} \textbf{0.8569} & \cellcolor{kbgH} 0.5106 
& \cellcolor{kbgH} 0.5093 & \cellcolor{kbgH} \textbf{0.6817}
& \cellcolor{kbgH} 0.5039 & \cellcolor{kbgH} 0.4869
% & 8
\\
\midrule
% \midrule[1pt]
% \multicolumn{12}{c}{\cellcolor{bglight} \textbf{Foundation Model:} \optlarge} \\
% \midrule[1pt]

\multirow{3}{*}{\optlarge}
& \cellcolor{kbgB} 0.5338 & \cellcolor{kbgB} 0.5236 
& \cellcolor{kbgB} 0.5042 & \cellcolor{kbgB} 0.4994 
& \cellcolor{kbgB} 0.5650 & \cellcolor{kbgB} 0.5174 
& \cellcolor{kbgB} \textbf{0.5026} & \cellcolor{kbgB} 0.3825 
& \cellcolor{kbgB} 0.5205 & \cellcolor{kbgB} 0.5026 
% & 2 \\
\\

& \cellcolor{kbgG} 0.5996 & \cellcolor{kbgG} 0.6165 
& \cellcolor{kbgG} 0.5189 & \cellcolor{kbgG} 0.5181 
& \cellcolor{kbgG} 0.7002 & \cellcolor{kbgG} \textbf{0.6156} 
& \cellcolor{kbgG} 0.4853 & \cellcolor{kbgG} \textbf{0.7665} 
& \cellcolor{kbgG} \textbf{0.5446} & \cellcolor{kbgG} \textbf{0.5037} 
% & 40 \\
\\

& \cellcolor{kbgH} \textbf{0.7259} & \cellcolor{kbgH} \textbf{0.8132} 
& \cellcolor{kbgH} \textbf{0.5374} & \cellcolor{kbgH} \textbf{0.6220}
& \cellcolor{kbgH} \textbf{0.8658} & \cellcolor{kbgH} 0.5813 
& \cellcolor{kbgH} 0.5014 & \cellcolor{kbgH} 0.6959 
& \cellcolor{kbgH} 0.5248 & \cellcolor{kbgH} 0.4951 
% & 38 \\
\\
\midrule
% \midrule[1pt]
% \multicolumn{12}{c}{\cellcolor{bglight} \textbf{Foundation Model:} \llamasan} \\
% \midrule[1pt]
% \rB{}

\multirow{3}{*}{\llamasan}
& \cellcolor{kbgB} 0.4904 & \cellcolor{kbgB} 0.6412 
& \cellcolor{kbgB} 0.5577 & \cellcolor{kbgB} 0.5191 
& \cellcolor{kbgB} 0.7690 & \cellcolor{kbgB} 0.5267
& \cellcolor{kbgB} 0.5136 & \cellcolor{kbgB} 0.5454 
& \cellcolor{kbgB} 0.5223 & \cellcolor{kbgB} 0.5342 
% & 5 \\
\\
% \rG{} 
& \cellcolor{kbgG} 0.6732 & \cellcolor{kbgG} 0.6223 
& \cellcolor{kbgG} 0.5864 & \cellcolor{kbgG} 0.5626 
& \cellcolor{kbgG} 0.7295 & \cellcolor{kbgG} \textbf{0.7203} 
& \cellcolor{kbgG} 0.5764 & \cellcolor{kbgG} \textbf{0.7828} 
& \cellcolor{kbgG} \textbf{0.6296} & \cellcolor{kbgG} \textbf{0.5806} 
% & 62 \\
\\
& \cellcolor{kbgH} \textbf{0.7206} & \cellcolor{kbgH} \textbf{0.8235}
& \cellcolor{kbgH} \textbf{0.6660} & \cellcolor{kbgH} \textbf{0.6281} 
& \cellcolor{kbgH} \textbf{0.8524} & \cellcolor{kbgH} 0.6683
& \cellcolor{kbgH} \textbf{0.5846} & \cellcolor{kbgH} 0.7042
& \cellcolor{kbgH} 0.6139 & \cellcolor{kbgH} 0.5318
\\
% & 48 \\
% \midrule[1pt]
% \multicolumn{11}{c}{\cellcolor{bglight} \textbf{Recommendation Approach:} Embedding-based} \\
% \midrule[1pt]

% \multirow{3}{*}{\bertbase}
% & \cellcolor{kbgB} 0.5263 
% & \cellcolor{kbgB} 0.5305 
% & \cellcolor{kbgB} 0.5160 
% & \cellcolor{kbgB} 0.5139 
% & \cellcolor{kbgB} 0.5167 
% & \cellcolor{kbgB} 0.4978 
% & \cellcolor{kbgB} 0.5123 
% & \cellcolor{kbgB} 0.5609 
% & \cellcolor{kbgB} 0.5257 
% & \cellcolor{kbgB} 0.5137 
% & 2 \\
% & \cellcolor{kbgG} 0.5011 
% & \cellcolor{kbgG} 0.5055 
% & \cellcolor{kbgG} 0.5159 
% & \cellcolor{kbgG} 0.5245 
% & \cellcolor{kbgG} 0.4879 
% & \cellcolor{kbgG} 0.5779 
% & \cellcolor{kbgG} 0.5035 
% & \cellcolor{kbgG} 0.4585 
% & \cellcolor{kbgG} 0.4885 
% & \cellcolor{kbgG} 0.4939 
% & 26 \\

% \\
% \midrule
% \multirow{3}{*}{\optlarge}
% & \cellcolor{kbgB} 0.5510 
% & \cellcolor{kbgB} 0.5447 
% & \cellcolor{kbgB} 0.5258 
% & \cellcolor{kbgB} 0.5137 
% & \cellcolor{kbgB} 0.6370 
% & \cellcolor{kbgB} 0.5303 
% & \cellcolor{kbgB} 0.5289 
% & \cellcolor{kbgB} 0.7989 
% & \cellcolor{kbgB} 0.5130 
% & \cellcolor{kbgB} 0.5127 
% & 6
% \\
% & \cellcolor{kbgG} 0.4863
% & \cellcolor{kbgG} 0.4859 
% & \cellcolor{kbgG} 0.5095
% & \cellcolor{kbgG} 0.5049
% & \cellcolor{kbgG} 0.5452
% & \cellcolor{kbgG} 0.5813
% & \cellcolor{kbgG} 0.4828
% & \cellcolor{kbgG} 0.6611
% & \cellcolor{kbgG} 0.4926
% & \cellcolor{kbgG} 0.5217
% & 330 \\
% \\
% \midrule
% \multirow{3}{*}{\llamasan}
% & 0.5666 
% & 0.5218 
% & 0.5150 
% & 0.5162 
% & 0.6487 
% & 0.4985 
% & 0.5212 
% & 0.6900 
% & 0.5189 
% & 0.5061 
% \\ 
% \\
% \\
\bottomrule
\end{tabular}
}
\end{table*}


% \begin{table*}[ht]
% \centering
% \renewcommand{\arraystretch}{1.2} 

% \setlength\tabcolsep{3pt}

% \caption{Ablation Studies.}\label{tab:zero-text}

% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|lllllllllll}
% \toprule
% Fine-tune & \mind{} & \microlens{} & \goodreads{} & \cds{} & \hm{} & \movielens{} & \yelp{} & \steam{} & \electronics{} & \hotelrec{} & Overall \\

% \midrule[1pt]
% \multicolumn{12}{c}{\cellcolor{bglight} \textbf{Foundation Model:} \bertbase} \\
% \midrule[1pt]
% \rB{} 
% & \cellcolor{kbgB} 0.4963 & \cellcolor{kbgB} 0.4992 
% & \cellcolor{kbgB} 0.4958 & \cellcolor{kbgB} 0.5059 
% & \cellcolor{kbgB} 0.5204 & \cellcolor{kbgB} 0.4934 
% & \cellcolor{kbgB} 0.4914 & \cellcolor{kbgB} 0.5002 
% & \cellcolor{kbgB} 0.5037 & \cellcolor{kbgB} 0.4955 
% & \cellcolor{kbgB} 0.5002 
% \\

% \rG{}
% & 0.6004 & 0.5711 & 0.5213 & 0.5092 & 0.6607 
% & 0.5675 & 0.5218 & 0.6189 & 0.5091 & 0.4795
% \\

% \rH{}
% & 0.7004 & 0.8019 & 0.5648 & 0.5653 & 0.8569
% & 0.5106 & 0.5093 & 0.6817 & 0.5039 & 0.4869
% \\

% \midrule
% \pog{} 
% & \cellcolor{kbgD} 0.5164 & \cellcolor{kbgF} 0.5669 
% & \cellcolor{kbgF} 0.5119 & \cellcolor{kbgF} 0.5050 
% & \cellcolor{kbgF} 0.6242 & \cellcolor{kbgF} 0.5118 
% & \cellcolor{kbgF} 0.4975 & \cellcolor{kbgF} 0.6418 
% & \cellcolor{kbgF} 0.5265 & \cellcolor{kbgF} 0.4850 
% & \cellcolor{kbgF} 0.5387 \\

% \pens{} 
% & \cellcolor{kbgF} 0.6067 & \cellcolor{kbgD} 0.5781 
% & \cellcolor{kbgF} 0.5181 & \cellcolor{kbgF} 0.5027 
% & \cellcolor{kbgF} 0.6849 & \cellcolor{kbgF} 0.5085 
% & \cellcolor{kbgF} 0.4913 & \cellcolor{kbgF} 0.7405 
% & \cellcolor{kbgF} 0.5147 & \cellcolor{kbgF} 0.4842 
% & \cellcolor{kbgF} 0.5630 \\

% \netflix{} 
% & \cellcolor{kbgF} 0.5865 & \cellcolor{kbgF} 0.5459 
% & \cellcolor{kbgD} 0.5105 & \cellcolor{kbgF} 0.5076 
% & \cellcolor{kbgF} 0.6664 & \cellcolor{kbgF} 0.5829 
% & \cellcolor{kbgF} 0.4964 & \cellcolor{kbgF} 0.6971 
% & \cellcolor{kbgF} 0.5272 & \cellcolor{kbgF} 0.5010 
% & \cellcolor{kbgF} 0.5622 \\

% \books{} 
% & \cellcolor{kbgF} 0.5585 & \cellcolor{kbgF} 0.5415 
% & \cellcolor{kbgF} 0.5258 & \cellcolor{kbgD} 0.5141 
% & \cellcolor{kbgF} 0.6086 & \cellcolor{kbgF} 0.5418 
% & \cellcolor{kbgF} 0.5024 & \cellcolor{kbgF} 0.6162 
% & \cellcolor{kbgF} 0.5131 & \cellcolor{kbgF} 0.4937 
% & \cellcolor{kbgF} 0.5416 \\

% \lastfm{} 
% & \cellcolor{kbgF} 0.5378 & \cellcolor{kbgF} 0.5561 
% & \cellcolor{kbgF} 0.5200 & \cellcolor{kbgF} 0.5059 
% & \cellcolor{kbgD} 0.6262 & \cellcolor{kbgF} 0.5613 
% & \cellcolor{kbgF} 0.4827 & \cellcolor{kbgF} 0.6111 
% & \cellcolor{kbgF} 0.5083 & \cellcolor{kbgF} 0.4687 
% & \cellcolor{kbgF} 0.5378 \\

% \midrule

% \netflix{} 
% & \cellcolor{kbgF} 0.5396
% & \cellcolor{kbgD} 0.5328
% & \cellcolor{kbgF} 0.5080 
% & \cellcolor{kbgF} 0.5097
% & \cellcolor{kbgF} 0.6191
% & \cellcolor{kbgF} 0.5656
% & \cellcolor{kbgF} 0.5117
% & \cellcolor{kbgF} 0.6954
% & \cellcolor{kbgF} 0.5255
% & \cellcolor{kbgF} 0.5077
% \\

% \books{}
% & 0.5057 & 0.5331 & 0.5243 & 0.5019 & 0.5886 & 0.5336 & 0.5218 & 0.6142 & 0.5207 & 0.5076 \\

% \pens{}
% & 0.6066 & 0.5617 & 0.5243 & 0.5075 & 0.6450 & 0.5253 & 0.4980 & 0.7295 & 0.5242 & 0.4882 \\



% \midrule[1pt]
% \multicolumn{12}{c}{\cellcolor{bglight} \textbf{Foundation Model:} \optlarge} \\
% \midrule[1pt]

% \rB{}
% & \cellcolor{kbgB} 0.5338 & \cellcolor{kbgB} 0.5236 
% & \cellcolor{kbgB} 0.5042 & \cellcolor{kbgB} 0.4994 
% & \cellcolor{kbgB} 0.5650 & \cellcolor{kbgB} 0.5174 
% & \cellcolor{kbgB} 0.5026 & \cellcolor{kbgB} 0.3825 
% & \cellcolor{kbgB} 0.5205 & \cellcolor{kbgB} 0.5026 
% & \cellcolor{kbgB} 0.5052 \\

% \rC{}
% & \cellcolor{kbgC} 0.7344 & \cellcolor{kbgC} 0.7735 
% & \cellcolor{kbgC} 0.4985 & \cellcolor{kbgC} 0.5808 
% & \cellcolor{kbgC} 0.5155 & - & - & - & - & - & \\

% \rG{}

% & 0.5996 & 0.6165 & 0.5189 & 0.5181 & 0.7002 & 0.6156 & 0.4853 & 0.7665 & 0.5446 & 0.5037 \\

% \pog{} 
% & \cellcolor{kbgD} 0.5326 & \cellcolor{kbgF} 0.5142 
% & \cellcolor{kbgF} 0.5027 & \cellcolor{kbgF} 0.5023 
% & \cellcolor{kbgF} 0.5530 & \cellcolor{kbgF} 0.5142 
% & \cellcolor{kbgF} 0.5054 & \cellcolor{kbgF} 0.4195 
% & \cellcolor{kbgF} 0.5302 & \cellcolor{kbgF} 0.4988 
% & \cellcolor{kbgF} 0.5073 \\
% \pens{} 
% & \cellcolor{kbgF} 0.6311 & \cellcolor{kbgD} 0.5472 
% & \cellcolor{kbgF} 0.5330 & \cellcolor{kbgF} 0.5072 
% & \cellcolor{kbgF} 0.6894 & \cellcolor{kbgF} 0.5457 
% & \cellcolor{kbgF} 0.4703 & \cellcolor{kbgF} 0.8305 
% & \cellcolor{kbgF} 0.5280 & \cellcolor{kbgF} 0.4841 
% & \cellcolor{kbgF} 0.5767 \\
% \netflix{} 
% & \cellcolor{kbgF} 0.5996 & \cellcolor{kbgF} 0.6165 
% & \cellcolor{kbgD} 0.5189 & \cellcolor{kbgF} 0.5181 
% & \cellcolor{kbgF} 0.7002 & \cellcolor{kbgF} 0.6156 
% & \cellcolor{kbgF} 0.4853 & \cellcolor{kbgF} 0.7665 
% & \cellcolor{kbgF} 0.5446 & \cellcolor{kbgF} 0.5037 
% & \cellcolor{kbgF} 0.5869 \\
% \books{} 
% & \cellcolor{kbgF} 0.5492 & \cellcolor{kbgF} 0.6064 
% & \cellcolor{kbgF} 0.5141 & \cellcolor{kbgD} 0.5211 
% & \cellcolor{kbgF} 0.7029 & \cellcolor{kbgF} 0.6054 
% & \cellcolor{kbgF} 0.5167 & \cellcolor{kbgF} 0.6299 
% & \cellcolor{kbgF} 0.5286 & \cellcolor{kbgF} 0.5043 
% & \cellcolor{kbgF} 0.5679 \\
% \lastfm{} 
% & \cellcolor{kbgF} 0.5612 & \cellcolor{kbgF} 0.5979 
% & \cellcolor{kbgF} 0.5394 & \cellcolor{kbgF} 0.5016 
% & \cellcolor{kbgD} 0.7380 & \cellcolor{kbgF} 0.5982 
% & \cellcolor{kbgF} 0.4676 & \cellcolor{kbgF} 0.8405 
% & \cellcolor{kbgF} 0.5317 & \cellcolor{kbgF} 0.4772 
% & \cellcolor{kbgF} 0.5853 \\

% \midrule[1pt]
% \multicolumn{12}{c}{\cellcolor{bglight} \textbf{Foundation Model:} \llamasan} \\
% \midrule[1pt]
% \rB{}
% & \cellcolor{kbgB} 0.4904 & \cellcolor{kbgB} 0.6412 
% & \cellcolor{kbgB} 0.5577 & \cellcolor{kbgB} 0.5191 
% & \cellcolor{kbgB} 0.7690 & \cellcolor{kbgB} 0.5267
% & \cellcolor{kbgB} 0.5136 & \cellcolor{kbgB} 0.5454 
% & \cellcolor{kbgB} 0.5223 & \cellcolor{kbgB} 0.5342 \\
% \rG{} 
% & \cellcolor{kbgG} 0.6732 & \cellcolor{kbgG} 0.6223 
% & \cellcolor{kbgG} 0.5864 & \cellcolor{kbgG} 0.5626 
% & \cellcolor{kbgG} 0.7295 & \cellcolor{kbgG} 0.7203 
% & \cellcolor{kbgG} 0.5764 & \cellcolor{kbgG} 0.7828 
% & \cellcolor{kbgG} 0.6296 & \cellcolor{kbgG} 0.5806 
% & \cellcolor{kbgG} 0.6464 \\
% \midrule
% \books{}
% & \cellcolor{kbgF} 0.5040 
% & \cellcolor{kbgF} 0.5322
% & \cellcolor{kbgF} 0.5876 
% & \cellcolor{kbgF} 0.5600 
% & \cellcolor{kbgF} 0.5750 
% & \cellcolor{kbgF} 0.6935
% & \cellcolor{kbgF} 0.5727 
% & \cellcolor{kbgF} 0.6373
% & \cellcolor{kbgF} 0.6267 
% & \cellcolor{kbgF} 0.6149 \\
% \lastfm{}
% & 0.5785 & 0.6462 & 0.5864 & 0.5039 & 0.7444 & 0.6843 & 0.5089 & 0.9307 & 0.5506 & 0.5216 & \\
% \netflix{}
% & 0.5377 & 0.6044 & 0.5831 & 0.5348 & 0.7175 & 0.7502 & 0.5072 & 0.8969 & 0.6004 & 0.5748 & \\

% \midrule
% \pog{} 
% & 0.4912 & 0.5175 & 0.5068 & 0.5011 & 0.5922
% & 0.5354 & 0.5147 & 0.5684 & 0.4896  & 0.5142
% \\
% \pens{}
% & 0.6713 & 0.6644 & 0.5427 & 0.5061 & 0.7069 
% & 0.5947 & 0.5075 & 0.8763 & 0.5179 & 0.4872 
% \\
% \netflix{}
% & 0.6052 & 0.6132 & 0.5635 & 0.5223 & 0.7198 
% & 0.7552 & 0.4837 & 0.8842 & 0.5578 & 0.5723
% \\
% \books{}
% & 0.5434 & 0.5519 & 0.5914 & 0.5505 & 0.6175 
% & 0.7205 & 0.5546 & 0.6796 & 0.6230 & \\

% \bottomrule
% \end{tabular}
% }
% \end{table*}

==> Tables/ablation-embed.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Ablation Studies.}\label{tab:zero-text}

\begin{tabular}{llllllllllll}
\toprule
Order & MIND & MovieLens & MicroLens & Goodreads & Yelp & Steam & CDs & H\&M & Electronics & HotelRec & Overall \\
\midrule
BERT$_\text{base}$-zst &
0.5263 & 0.4978 & 0.5305 & 0.5160 & 0.5123 & 0.5609 & 0.5139 & 0.5167 & 0.5257 & 0.5137 & 0.5214 \\
BERT$_\text{base}$-sft & 
0.6837 & - & 0.7671 & 0.5738 & - & - & 0.5909 & 0.8359 & - & - \\
BERT$_\text{base-1}$ & 0.5038 & 0.5039 & 0.5102 & 0.4925 & 0.5182 & 0.5307 & 0.5909 & 0.5222 & 0.5024 & 0.4950 & 0.5170 \\
BERT$_\text{base-2}$ & 0.5793 & 0.5060 & 0.4875 & 0.4995 & 0.5009 & 0.5386 & 0.5449 & 0.5066 & 0.5009 & 0.5140 & 0.5178 \\
BERT$_\text{base-3}$ & 0.5502 & 0.5743 & 0.4951 & 0.4994 & 0.4941 & 0.4056 & 0.5329 & 0.4775 & 0.5251 & 0.5059 & 0.5060 \\
BERT$_\text{base-4}$ & 0.5268 & 0.5174 & 0.5034 & 0.5096 & 0.5187 & 0.4315 & 0.5197 & 0.4591 & 0.4934 & 0.4977 & 0.4977 \\
BERT$_\text{base-5}$ & 0.4679 & 0.4910 & 0.5148 & 0.5073 & 0.4855 & 0.4748 & 0.5042 & 0.5132 & 0.4641 & 0.5024 & 0.4925 \\
BERT & 0.5011 & 0.5779 & 0.5055 & 0.5159 & 0.5035 & 0.4585 & 0.5245 & 0.4879 & 0.4885 & 0.4939 & 0.5057 \\
\midrule

OPT$_\text{large}$-zst &
0.5510 & 0.5303 & 0.5447 & 0.5258 & 0.5289 & 0.7989 & 0.5137 & 0.6370 & 0.5130 & 0.5127 & 0.5656 \\
OPT$_\text{large}$-sft & 
0.6788 & - & 0.7545 & 0.5754 & - & - & 0.5713 & 0.8163 & - & - \\
OPT$_\text{large}$-1 & 0.5106 & 0.5296 & 0.5133 & 0.4841 & 0.5108 & 0.5859 & 0.4873 & 0.5241 & 0.4518 & 0.5329 & 0.5130 \\
OPT$_\text{large}$ & 0.4863 & 0.5813 & 0.4859 & 0.5095 & 0.4828 & 0.6611 & 0.5049 & 0.5452 & 0.4926 & 0.5217 & 0.5271\\
\midrule
Llama-3$_\text{7B}$ & 0.6745 & \\
\end{tabular}
\end{table*}

==> Tables/ablation.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Ablation Studies.}\label{tab:zero-text}

\begin{tabular}{llllllllllll}
\toprule
Order & MIND & MovieLens & MicroLens & Goodreads & Yelp & Steam & CDs & H\&M & Electronics & HotelRec & Overall \\
\midrule
BERT$_\text{base}$-zst &
0.4963 & 0.4934 & 0.4992 & 0.4958 & 0.4914 & 0.5002 & 0.5059 & 0.5204 & 0.5037 & 0.4955 & 0.5002 \\
BERT$_\text{base}$-sft & 0.7118 & - & 0.8148 & 0.5208 & - & - & 0.6185 & 0.8701 & - & - \\ 
BERT$_\text{base-1}$ & 
0.5164 & 0.5118 & 0.5669 & 0.5119 & 0.4975 & 0.6418 & 0.5050 & 0.6242 & 0.5265 & 0.4850 & 0.5387 \\
BERT$_\text{base-2}$ & 
0.6067 & 0.5085 & 0.5781 & 0.5181 & 0.4913 & 0.7405 & 0.5027 & 0.6849 & 0.5147 & 0.4842 & 0.5630 \\
BERT$_\text{base-3}$ & 
0.5865 & 0.5829 & 0.5459 & 0.5105 & 0.4964 & 0.6971 & 0.5076 & 0.6664 & 0.5272 & 0.5010 & 0.5622 \\
BERT$_\text{base-4}$ & 
0.5585 & 0.5418 & 0.5415 & 0.5258 & 0.5024 & 0.6162 & 0.5141 & 0.6086 & 0.5131 & 0.4937 & 0.5416 \\
BERT$_\text{base-5}$ & 
0.5378 & 0.5613 & 0.5561 & 0.5200 & 0.4827 & 0.6111 & 0.5059 & 0.6262 & 0.5083 & 0.4687 & 0.5378 \\
\midrule
OPT$_\text{large}$-zst &
0.5338 & 0.5174 & 0.5236 & 0.5042 & 0.5026 & 0.3825 & 0.4994 & 0.5650 & 0.5205 & 0.5026 & 0.5052 \\
OPT$_\text{large}$-sft &
0.7344 & - & 0.7735 & 0.4985 & - & - & 0.5808 & 0.5155 & - & - \\
OPT$_\text{large-1}$ &
0.5326 & 0.5142 & 0.5142 & 0.5027 & 0.5054 & 0.4195 & 0.5023 & 0.5530 & 0.5302 & 0.4988 & 0.5073 \\
OPT$_\text{large-2}$ & 
0.6311 & 0.5457 & 0.5472 & 0.5330 & 0.4703 & 0.8305 & 0.5072 & 0.6894 & 0.5280 & 0.4841 & 0.5767 \\
OPT$_\text{large-3}$ & 
0.5996 & 0.6156 & 0.6165 & 0.5189 & 0.4853 & 0.7665 & 0.5181 & 0.7002 & 0.5446 & 0.5037 & 0.5869 \\
OPT$_\text{large-4}$ & 
0.5492 & 0.6054 & 0.6064 & 0.5141 & 0.5167 & 0.6299 & 0.5211 & 0.7029 & 0.5286 & 0.5043 & 0.5679 \\
OPT$_\text{large-5}$ & 
0.5612 & 0.5982 & 0.5979 & 0.5394 & 0.4676 & 0.8405 & 0.5016 & 0.7380 & 0.5317 & 0.4772 & 0.5853 \\
\midrule
Llama-3 & 
0.6732 & 0.7203 & 0.6223 & 0.5864 & 0.5764 & 0.7828 & 0.5626 & 0.7295 & 0.6296 & 0.5806 & 0.6464 \\
\midrule
Llama-3$_{-1}$ & 
0.4982 & 0.5381 & 0.5010 & 0.5077 & 0.4823 & 0.5677 & 0.5019 & 0.5803 & 0.4987\\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/baseline.tex <==
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Recommendation ability across traditional recommenders, zero-shot language model based recommenders, and tuned language model based recommenders in single domain recommendation scenario.}\label{tab:single-domain}

\begin{tabular}{lllllll}
\toprule
 & MIND & MicroLens & Goodreads & CDs & H\&M & Overall \\
\midrule
DeepFM & 0.6670 & 0.7594 & 0.6671 & 0.5681 & 0.7013 & \\
DCNv2 & 0.6707 & 0.7578 & 0.5778 & 0.5664 & 0.7076 & \\
FinalMLP & 0.6649 & 0.7600 & 0.5807 & 0.5670 & 0.7086 & \\
DIN & 0.6794 & 0.7587 & 0.6794 & 0.5683 & 0.7091 & \\

 
\bottomrule
\end{tabular}
\end{table}

==> Tables/dataset-list.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Datasets evaluated or finetuned in our benchmark.}\label{tab:dataset-list}

\resizebox{\linewidth}{!}{
\begin{tabular}{lllllllll}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Type}} & \multicolumn{3}{l}{\textbf{Test set}} & \multicolumn{3}{l}{\textbf{Finetune set}} & \multirow{2}{*}{\textbf{Provider}} \\
% & \multirow{2}{*}{Source} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 &  & \#Sample & \#Item & \#User & \#Sample & \#Item & \#User & \\
\midrule
H\&M & Fashion & 20,000 & 15,305 & 5,000 & 100,000 & 50,319 & 25,000 & H\&M \\
% & \url{https://s.6-79.cn/to77vc} \\
% \url{https://www.kaggle.com/competitions/h-and-m-personalized-fashion-recommendations} \\
MIND & News & 20,006 & 3,088 & 1,514 & 100,000 & 5,481 & 7,606 & Microsoft \\
% & \url{https://s.6-79.cn/k2Susd} \\
% \url{https://msnews.github.io/} \\
MicroLens & Video & 20,000 & 11,073 & 5,000 & 100,000 & 18,658 & 25,000 &  Westlake Uni. \\
% & \url{https://s.6-79.cn/QRqTfh} \\
% \url{https://github.com/westlake-repl/MicroLens} \\
Goodreads & Book & 20,009 & 12,984 & 1,736 & 100,005 & 40,322 & 8,604 &  UCSD \\
% & \url{https://s.6-79.cn/D8WmWj} \\
% \url{https://mengtingwan.github.io/data/goodreads} \\
CDs & Music & 20,003 & 15,568 & 4,930 & 100,003 & 55,428 & 24,618 & Amazon \\
% & \url{https://s.6-79.cn/F2ftHB} \\
% \url{https://cseweb.ucsd.edu/~jmcauley/datasets/amazon_v2/} \\
\midrule
MovieLens & Movie & 20,008 & 4,300 & 2,251 & -  & - & - & UMN \\
% & \url{https://s.6-79.cn/T1aP1f} \\
% \url{https://grouplens.org/datasets/movielens/} \\
Yelp & Restaurant & 20,003 & 15,239 & 4,013 & - & - & - &  Yelp \\
% & \url{https://s.6-79.cn/BrqJ12} \\
% \url{https://www.yelp.com/dataset/} \\
Steam & Game & 20,000 & 2,216 & 5,000 & - & - & - &  OPI PIB \\
% & \url{https://s.6-79.cn/2YVdKq} \\
% \url{https://github.com/YangLiangwei/SCGRec?tab=readme-ov-file} \\
Electronics & E-commerce & 20,002 & 11,045 & 5,431 & - & - & - &  Amazon \\
% & \url{https://s.6-79.cn/tvFDoU} \\
% \url{https://cseweb.ucsd.edu/~jmcauley/datasets/amazon_v2/} \\
HotelRec & Hotel & 20,002 & 17,295 & 5,437 & - & - & - &  EPFL \\
% & \url{https://s.6-79.cn/xL3RDk} \\
% \url{https://www.dropbox.com/s/ltr0010rhths2zi/Full_HotelRec.zip?dl=0}\\
\midrule
POG & Fashion & - & - & - & 100,002 & 15,846 & 15,734 & Alibaba \\
% & \url{https://s.6-79.cn/MRlqve} \\
% \url{https://drive.google.com/drive/folders/1tHCG8x1fLF18ccuXMJsEB8mNIn5n4F2l?usp=sharing} \\
PENS & News & - & - & - & 100,007 & 9,053 & 8,542 & Microsoft \\
% & \url{https://s.6-79.cn/6jysPT} \\
% \url{https://msnews.github.io/pens_data.html} \\
Netflix & Video & - & - & - & 100,010 & 3,645 & 13,424 & Netflix \\
% & \url{https://s.6-79.cn/ieDyxv} \\
% \url{https://www.kaggle.com/datasets/netflix-inc/netflix-prize-data} \\
Books & Book & - & - & - & 100,002 & 28,471 & 25,139 & Amazon \\
% & \url{https://s.6-79.cn/9mdMXe} \\
% \url{https://cseweb.ucsd.edu/~jmcauley/datasets/amazon_v2/} \\
LastFM & Music & - & - & - & 100,100 & 94,319 & 910 & LastFM \\
% & \url{https://s.6-79.cn/ryAnFq} \\
% \url{http://millionsongdataset.com/lastfm} \\
\bottomrule
\end{tabular}
}
\end{table*}


==> Tables/llm-list.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Large language and recommendation models benchmarked in our paper.}\label{tab:llm-list}

\begin{tabular}{lllll}
\toprule
Date & Model & Size (M) & Institution & Source \\
\midrule
2018.10 & BERT$_\text{base}$ & 110 & Google & \url{https://huggingface.co/google-bert/bert-base-uncased} \\
2022.05 & OPT$_\text{base}$ & 331 & Meta & \url{https://huggingface.co/facebook/opt-350m} \\
2022.05 & OPT$_\text{large}$ & 1,316 & Meta & \url{https://huggingface.co/facebook/opt-1.3b} \\
2022.11 & GPT-3.5 & - & OpenAI & \url{https://platform.openai.com/docs/guides/text-generation} \\
2023.02 & Llama-1 & 6,738 & Meta & \url{https://huggingface.co/huggyllama/llama-7b} \\
2023.03 & GPT-4 & - & OpenAI & \url{https://platform.openai.com/docs/guides/text-generation} \\
2023.05 & E5-2 & 109 & Microsoft & \url{https://huggingface.co/intfloat/e5-base-v2} \\
2023.06 & Claude-2 & - & Anthropic & \url{https://docs.anthropic.com/en/api/complete} \\
2023.06 & Llama-2 & 6,738 & Meta & \url{https://github.com/meta-llama/llama3} \\
% 2023.09 & BGE-1.5 & 110 & BAAI & \url{https://huggingface.co/BAAI/bge-base-en-v1.5} \\
2023.10 & Phi-2 & 2,780 & Microsoft & \url{https://huggingface.co/microsoft/phi-2} \\
2024.01 & GLM-4 & 9,400 & THU & \url{https://huggingface.co/THUDM/glm-4-9b-chat} \\
2024.02 & Mistral-2 & 7,248 & MistralAI & \url{https://huggingface.co/mistralai/Mistral-7B-Instruct-v0.3} \\
2024.04 & Llama-3 & 8,030 & Meta & \url{https://huggingface.co/meta-llama/Llama-2-7b-hf} \\
2024.06 & Qwen-2 & 7,616 & Alibaba & \url{https://huggingface.co/Qwen/Qwen2-7B-Instruct} \\
% 2023 & Phi-3 & 7B & Microsoft & \url{https://huggingface.co/microsoft/Phi-3-small-8k-instruct} \\
\midrule
2022.03 & P5 & 223 & Rutgers. & \url{https://huggingface.co/makitanikaze/P5} \\
2023.05 & Recformer & 148 & UCSD & \url{https://github.com/AaronHeee/RecFormer} \\
\bottomrule
\end{tabular}

\end{table*}


==> Tables/sft.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Recommendation ability with large language model supervised finetuning}\label{tab:sft}

\begin{tabular}{llllllllllll}
\toprule
 & MIND & MovieLens & MicroLens & Goodreads & Yelp & Steam & CDs & H\&M & Electronics & HotelRec & Overall \\
\midrule
OPT$_\text{large}$ &
&  &  &  &  &  &  &  &  &  \\
Llama-1 &
&  &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/training.tex <==
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Finetuning details.}\label{tab:finetune}

\begin{tabular}{llllllllll}
\toprule
Backbone & LoRA & BZ & LR & Order & Dataset & Train & Valid & Epoch & Signature \\
\midrule
BERT$_\text{base}$ & 32-128-0.1 & 64 & 5e-4 & 1 & POG &  &  & 8 & @572957 \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-5 & 2 & PENS &  &  & 10 & @c5ab28 \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 3 & Netflix &  &  & 6 & @640c3d \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 4 & Books &  &  & 10 & @25ef56 \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 5 & LastFM &  &  & 7 & @177d18 \\
\midrule
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-5 & 1 & POG & & & 2 & @0a2117 \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-5 & 2 & PENS & & & 9 & @ac933a \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-5 & 3 & Netflix & & & 6 & @965058 \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-5 & 4 & Books & & & 10 & @87f5f8 \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-5 & 5 & LastFM & & & 1 & @de396b \\
\midrule
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 1 & POG &  & & 12 & @1f18d2 \\
\midrule
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 1 & MIND &  & & 3 & @eafc62 \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 1 & MicroLens &  & & 9 & @e93b4e \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 1 & Goodreads &  & & 4 & @1b6d57 \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 1 & H\&M &  & & 11 & @02b877 \\
BERT$_\text{base}$ & 32-128-0.1 & 64 & 1e-4 & 1 & CDs &  & & 7 & @fdcaef \\
\midrule
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-4 & 1 & MIND & & & 2 & @27a5e9 \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-4 & 1 & MicroLens & & & 1 & @bdcdec \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-4 & 1 & Goodreads & & & 4 & @f0ec3f \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-4 & 1 & CDs & & & 7 & @b01190 \\
OPT$_\text{large}$ & 32-128-0.1 & 24 & 1e-4 & 1 & H\&M & & & 7 & @138d1e \\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/zero-embed.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Zero-shot recommendation ability with embedding extraction.}\label{tab:zero-embed}

\begin{tabular}{llllllllllll}
\toprule
& MIND & MovieLens & MicroLens & Goodreads & Yelp & Steam & CDs & H\&M & Electronics & HotelRec & Overall \\
% & \rotatebox{45}{MIND} & \rotatebox{45}{MovieLens} & \rotatebox{45}{MicroLens} & \rotatebox{45}{Goodreads} & \rotatebox{45}{Yelp} & \rotatebox{45}{Steam} & \rotatebox{45}{CDs} & \rotatebox{45}{H\&M} & \rotatebox{45}{Electronics} & \rotatebox{45}{HotelRec} & \rotatebox{45}{Overall} \\
\midrule
BERT$_\text{base}$ &
0.5263 & 0.4978 & 0.5305 & 0.5160 & 0.5123 & 0.5609 & 0.5139 & 0.5167 & 0.5257 & 0.5137 & 0.5214 \\
OPT$_\text{base}$ &
0.5416 & 0.4914 & 0.5567 & 0.5290 & 0.5288 & 0.7462 & 0.5197 & 0.5334 & 0.5125 & 0.5078 & 0.5467 \\
OPT$_\text{large}$ &
0.5510 & 0.5303 & 0.5447 & 0.5258 & 0.5289 & 0.7989 & 0.5137 & 0.6370 & 0.5130 & 0.5127 & 0.5656 \\
Llama-1 &
0.5267 & 0.5352 & 0.5234 & 0.5063 & 0.4946 & 0.6298 & 0.5072 & 0.5832 & 0.5192 & 0.5044 & 0.5330 \\
Llama-2 & 
0.5291 & 0.4876 & 0.5251 & 0.5117 & 0.4997 & 0.5369 & 0.5165 & 0.4970 & 0.5228 & 0.5064 & 0.5133 \\
Llama-3 & 
0.5666 & 0.4985 & 0.5218 & 0.5150 & 0.5212 & 0.6900 & 0.5162 & 0.6487 & 0.5189 & 0.5061 & 0.5503 \\ 
Llama-3.1 & 
0.5682 & 0.4622 & 0.5247 & 0.5177 & 0.5182 & 0.6851 & 0.5109 & 0.6437 & 0.5274 & 0.5058 & 0.5464 \\
Mistral & 
0.5607 & 0.4792 & 0.5329 & 0.5240 & 0.5142 & 0.7685 & 0.5198 & 0.6051 & 0.5177 & 0.5123 & 0.5534 \\
GLM-4 & 
0.5179 & 0.5030 & 0.5362 & 0.5173 & 0.5211 & 0.7049 & 0.5173 & 0.6442 & 0.5180 & 0.5071 & 0.5487 \\
Qwen-2 & 
0.5347 & 0.4754 & 0.5391 & 0.5190 & 0.5106 & 0.6790 & 0.5212 & 0.6201 & 0.5213 & 0.5164 & 0.5437 \\
% Phi-3 & 0.6188 & 0.6614 &  & 0.5566 &  &  &  &  &  &  \\
Qwen0.5B & 0.5474 & 0.4519 & 0.5324 & 0.5135 & 0.5209 & 0.6134 & 0.5137 & 0.5916 & 0.5222 & 0.4974 \\
Qwen1.5B & 0.5395 & 0.4903 & 0.5397 & 0.5241 & 0.5091 & 0.6835 & 0.5097 & 0.6125 & 0.5240 & 0.5118\\
DeepseekQwen & 0.5211 & 0.4708 & 0.5293 & 0.5226 & 0.4952 & 0.5588 & 0.5110 & 0.4760 & 0.5089 & 0.5014 \\
Phi-2 & 
0.5381 & 0.5333 & 0.5364 & 0.5224 & 0.5093 & 0.7294 & 0.5167 & 0.5928 & 0.5208 & 0.5101 & 0.5509 \\
E5-2 &
0.6010 & 0.5062 & 0.6315 & 0.5217 & 0.4806 & 0.8221 & 0.5030 & 0.6569 & 0.5237 & 0.4788 & 0.5725 \\
\midrule
P5 &
0.5328 & 0.4791 & 0.5383 & 0.5046 & 0.4876 & 0.5802 & 0.5010 & 0.6049 & 0.5078 & 0.4931 & 0.5229 \\
Recformer &
0.5948 & 0.5421 & 0.6423 & 0.5186 & 0.5088 & 0.7329 & 0.5218 & 0.6781 & 0.5147 & 0.5262 & 0.5780 \\
RecGPT &
0.5129 & 0.5700 & 0.5160 & 0.5106 & 0.4949 & 0.6416 & 0.5209 & 0.5656 & 0.5066 & 0.5198 & 0.5359 \\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/zero-text.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} 

\caption{Zero-shot recommendation ability with answer generation.}\label{tab:zero-text}

\begin{tabular}{llllllllllll}
\toprule
 & MIND & MovieLens & MicroLens & Goodreads & Yelp & Steam & CDs & H\&M & Electronics & HotelRec & Overall \\
% & \rotatebox{45}{MIND} & \rotatebox{45}{MovieLens} & \rotatebox{45}{MicroLens} & \rotatebox{45}{Goodreads} & \rotatebox{45}{Yelp} & \rotatebox{45}{Steam} & \rotatebox{45}{CDs} & \rotatebox{45}{H\&M} & \rotatebox{45}{Electronics} & \rotatebox{45}{HotelRec} & \rotatebox{45}{Overall} \\
\midrule
BERT$_\text{base}$ &
0.4963 & 0.4934 & 0.4992 & 0.4958 & 0.4914 & 0.5002 & 0.5059 & 0.5204 & 0.5037 & 0.4955 & 0.5002 \\
OPT$_\text{base}$ &
0.5490 & 0.5104 & 0.4773 & 0.5015 & 0.5158 & 0.4257 & 0.5093 & 0.4555 & 0.5054 & 0.5028 & 0.4953\\
OPT$_\text{large}$ &
0.5338 & 0.5174 & 0.5236 & 0.5042 & 0.5026 & 0.3825 & 0.4994 & 0.5650 & 0.5205 & 0.5026 & 0.5052 \\
Llama-1 &
0.4583 & 0.6216 & 0.4572 & 0.4994 & 0.5206 & 0.5817 & 0.4995 & 0.4035 & 0.4892 & 0.5457 & 0.5077 \\
Llama-2 & 
0.4945 & 0.6030 & 0.4877 & 0.5273 & 0.5378 & 0.5622 & 0.5191 & 0.4519 & 0.4962 & 0.5305 & 0.5210 \\
Llama-3 &
0.4904 & 0.6412 & 0.5577 & 0.5191 & 0.5267 & 0.7690 & 0.5136 & 0.5454 & 0.5223 & 0.5342 & 0.5620 \\
Llama-3.1 &
0.5002 & 0.6444 & 0.5403 & 0.5271 & 0.5317 & 0.7650 & 0.5088 & 0.5462 & 0.5284 & 0.5268 & 0.5619 \\
Mistral & 
0.6300 & 0.6705 & 0.6579 & 0.5718 & 0.5187 & 0.8619 & 0.5230 & 0.7166 & 0.5205 & 0.4851 & 0.6156 \\
GLM-4 & 
0.6304 & 0.6568 & 0.6647 & 0.5671 & 0.5292 & 0.8556 & 0.5213 & 0.7319 & 0.5174 & 0.4961 & 0.6171 \\
Qwen-2$_\text{0.5B}$ & 0.4868 & 0.5153 & 0.5717 & 0.5148 & 0.5070 & 0.6372 & 0.5043 & 0.6287 & 0.5169 & 0.4985 \\
Qwen-2$_\text{1.5B}$ & 0.5411 & 0.5840 & 0.6072 & 0.5264 & 0.5392 & 0.8389 & 0.5174 & 0.6615 & 0.5258 & 0.5219 \\
Qwen-2$_\text{7B}$ & 
0.5862 & 0.6321 & 0.6640 & 0.5494 & 0.5317 & 0.8327 & 0.5256 & 0.7124 & 0.5202 & 0.5317 & 0.6086 \\
% Phi-3 &  &  &  &  &  &  &  & 0.7122 &  &  \\
DeepSeek & 0.5127 & 0.5389 & 0.5631 & 0.5165 & 0.5315 & 0.5858 & 0.5146 & 0.5994 & 0.5206 & 0.5149 \\
Phi-2 & 
0.4851 & 0.5296 & 0.5078 & 0.5049 & 0.5186 & 0.6061 & 0.4991 & 0.5447 & 0.5138 & 0.4986 & 0.5208 \\
GPT-3.5 & 
0.5057 & 0.5170 & 0.5110 & 0.5122 & 0.5039 & 0.6184 & 0.5046 & 0.5801 & 0.5134 & 0.5076 & 0.5274 \\
% GPT-4 & 0.5497 & OOM & OOM & OOM & OOM & OOM & OOM & OOM & OOM & OOM \\
% Claude-2 & 0.6172 & OOM & OOM & OOM & OOM & OOM & OOM & OOM & OOM & OOM \\
\midrule
RecGPT & 
0.5078 & 0.5069 & 0.4703 & 0.5083 & 0.5140 & 0.4924 & 0.5019 & 0.4875 & 0.5107 & 0.4937 & 0.4993 \\
P5 & 
0.4911 & 0.5138 & 0.5017 & 0.5027 & 0.5080 & 0.5296 & 0.5447 & 0.4845 & 0.5263 & 0.4905 & 0.5093 \\
% Recformer &  &  &  &  &  &  &  &  &  & \\
\midrule
% BERT$_\text{base}$ & 
% 0.6014 & 0.5073 & 0.9950 & 0.5165 & 0.5059 & 0.7125 & 0.5055 & 0.6995 & 0.5162 & 0.4815 & 0.6041 \\
% OPT$_\text{large}$ & 
% 0.5612 & 0.5982 & 0.9973 & 0.5394 & 0.4676 & 0.8405 & 0.5016 & 0.7380 & 0.5317 & 0.4772 & 0.6253 \\
Llama-3 & 
0.6732 & 0.7203 & 0.6223 & 0.5864 & 0.5764 & 0.7828 & 0.5626 & 0.7295 & 0.6296 & 0.5806 & 0.6464 \\
% \\
% OPT$_\text{large}$ &
% 0.5323 & 0.5213 & 0.6435 & 0.5060 & 0.5051 & 0.4117 & 0.5026 & 0.5551 & 0.5262 & 0.4984 & 0.5202 \\
BERT$_\text{base}$-Single & 0.7118 & - & 0.8148 & 0.5208 & - & - & 0.6185 & 0.8701 & - & - \\ 
\bottomrule
\end{tabular}
\end{table*}
